A Data-Adaptive Loss Function for Incomplete Data and Incremental Learning in Semantic Image Segmentation

In the last years, deep learning has dramatically improved the performances in a variety of medical image analysis applications. Among different types of deep learning models, convolutional neural networks have been among the most successful and they have been used in many applications in medical imaging. Training deep convolutional neural networks often requires large amounts of image data to generalize well to new unseen images. It is often time-consuming and expensive to collect large amounts of data in the medical image domain due to expensive imaging systems, and the need for experts to manually make ground truth annotations. A potential problem arises if new structures are added when a decision support system is already deployed and in use. Since the field of radiation therapy is constantly developing, the new structures would also have to be covered by the decision support system. In the present work, we propose a novel loss function, that adapts to the available data in order to utilize all available data, even when some have missing annotations. We demonstrate that the proposed loss function also works well in an incremental learning setting, where it can automatically incorporate new structures as they appear. Experiments on a large in-house data set show that the proposed method performs on par with baseline models, while greatly reducing the training time.

==> arXiv - 1st/glossaries.tex <==
\makeglossaries

\newacronym[plural=CNNs,firstplural=Convolutional Neural Networks (CNNs)]{cnn}{CNN}{Convolutional Neural Network}

\newacronym[plural=FCNs,firstplural=Fully Convolutional Networks (FCNs)]{fcn}{FCN}{Fully Convolutional Network}

\newacronym{ml}{ML}{machine learning}
\newacronym{dl}{DL}{deep learning}
\newacronym{qcmlb}{QC-MLB}{Question-Centric Multimodal Low-rank Bilinear}
\newacronym{bert}{BERT}{Bidirectional Encoder Representations from Transformers}
\newacronym{bleu}{BLEU}{Bilingual Evaluation Understudy}
\newacronym{mlm}{MLM}{Masked Language Model}
\newacronym{nsp}{NSP}{Next Sentence Prediction}
\newacronym{relu}{ReLU}{rectified linear unit}
\newacronym{lrelu}{LeakyReLU}{leaky rectified linear unit}
\newacronym{nn}{NN}{neural network}
\newacronym{mri}{MRI}{magnetic resonance imaging}

\newacronym{ct}{CT}{computed tomography}
\newacronym{t1c}{T1c}{post-contrast T1-weighted}
\newacronym{t2}{T2w}{T2-weighted}
\newacronym{t1}{T1w}{T1-weighted}
\newacronym{flair}{FLAIR}{T2  Fluid  Attenuated  Inversion  Recovery}
\newacronym{lgg}{LGG}{low-grade glioma}
\newacronym{hgg}{HGG}{high-grade glioma}

\newacronym{svm}{SVMs}{Support-vector Machines}
\newacronym{crf}{CRF}{Conditional Random Field}
\newacronym{vae}{VAE}{Variational Auto-Encoder}
\newacronym{tunet}{TuNet}{End-to-end Hierarchical Tumor Segmentation using Cascaded Networks}
\newacronym{dram}{DRAM}{dynamic random access memory}
% \newacronym{gpu}{GPU}{graphics processing unit}
% \newacronym{gpus}{GPUs}{graphics processing units}
\newacronym[plural=GPUs,firstplural=graphics processing units (GPUs)]{gpu}{GPU}{graphics processing unit}

\newacronym{hpc2n}{HPC2N}{High Performance Computer Center North}
\newacronym{snic}{SNIC}{Swedish National Infrastructure for Computing}

\newacronym{dsc}{DSC}{S{\o}rensen-Dice coefficient}
\newacronym{se}{SE}{standard error}
\newacronym{seb}{SEB}{Squeeze-and-Excitation block}
\newacronym[plural=REBs,firstplural=ResNet blocks]{res}{REB}{ResNet block}
\newacronym{hd}{HD}{Hausdorff distance}
\newacronym{hd95}{HD95}{$95^{th}$ percentile of the Hausdorff distance}
\newacronym{dauc}{DAUC}{Dice Area Under Curve}
\newacronym{rftp}{RFTPs}{Ratio of Filtered True Positives}
\newacronym{rftn}{RFTNs}{Ratio of Filtered True Negatives}

\newacronym[plural=SDs,firstplural=standard deviations (SDs)]{sd}{SD}{standard deviation}
\newacronym{brats}{BraTS 2020}{Brain Tumors in Multimodal Magnetic Resonance Imaging Challenge 2020}


\newacronym{mdnet}{MDNet}{End-to-end Multi-Decoder Cascaded Network for Tumor Segmentation}
\newacronym{ce}{CE}{categorical cross-entropy}

\newacronym{miccai}{MICCAI}{International Conference on Medical Image Computing and Computer Assisted Intervention}

\newacronym[plural=OARs,firstplural=organs-at-risks (OARs)]{oar}{OAR}{organs-at-risk}

\newacronym{loss}{loss}{Data-Adaptive Loss Function}

\newacronym{ravd}{RAVD}{relative absolute volume difference}
\newacronym{assd}{ASSD}{average symmetric surface distance}

\newacronym{dna}{DNA}{deoxyribonucleic acid}

\newacronym{asd}{ASD}{symmetric surface distance}
\newacronym{tpe}{TPE}{Tree-structured Parzen Estimator Approach}
\newacronym{rmse}{RMSE}{root mean square error}
\newacronym{ssl}{SSL}{semi-supervised learning}





 


